A diagrammatic approach to Hopf monads

Given a Hopf algebra in a symmetric monoidal category with duals, the category of modules inherits the structure of a monoidal category with duals. If the notion of algebra is replaced with that of monad on a monoidal category with duals then Bruguieres and Virelizier showed when the category of modules inherits this structure of being monoidal with duals, and this gave rise to what they called a Hopf monad. In this paper it is shown that there are good diagrammatic descriptions of dinatural transformations which allows the three-dimensional, object-free nature of their constructions to become apparent.

==> figs/fig2pstex <==
#! /bin/zsh -f
for fig in *.fig; do
  if [[ -e ../pstex/${fig:r}.eps && ../pstex/${fig:r}.eps -nt $fig ]]; then
	print "Skipping   ${fig:r}"
   else
        print "Processing ${fig:r}"
	print ${fig:r}
	fig2dev -L pstex  $fig ../pstex/${fig:r}.eps
	epstopdf ../pstex/${fig:r}.eps -o ../pstex/${fig:r}.pdf
	fig2dev -L pstex_t -F -p "\\figdir/${fig:r}" $fig ../pstex/${fig:r}.pstex_t
 fi
done


